Panda: Neighbor Discovery on a Power Harvesting Budget

Object tracking applications are gaining popularity and will soon utilize Energy Harvesting (EH) low-power nodes that will consume power mostly for Neighbor Discovery (ND) (i.e., identifying nodes within communication range). Although ND protocols were developed for sensor networks, the challenges posed by emerging EH low-power transceivers were not addressed. Therefore, we design an ND protocol tailored for the characteristics of a representative EH prototype: the TI eZ430-RF2500-SEH. We present a generalized model of ND accounting for unique prototype characteristics (i.e., energy costs for transmission/reception, and transceiver state switching times/costs). Then, we present the Power Aware Neighbor Discovery Asynchronously (Panda) protocol in which nodes transition between the sleep, receive, and transmit states. We analyze \name and select its parameters to maximize the ND rate subject to a homogeneous power budget. We also present Panda-D, designed for non-homogeneous EH nodes. We perform extensive testbed evaluations using the prototypes and study various design tradeoffs. We demonstrate a small difference (less then 2%) between experimental and analytical results, thereby confirming the modeling assumptions. Moreover, we show that Panda improves the ND rate by up to 3x compared to related protocols. Finally, we show that Panda-D operates well under non-homogeneous power harvesting.

==> tex/preamble.tex <==

%\subsection{Preamble Mode ($C_{\text{tx}}<C_{\text{rx}}$)}

In this case, we consider when the energy cost of transmitting is less than
that of listening ($C_{\text{tx}}>C_{\text{rx}}$). Here, since transmitting is
inexpensive, a node transmits a preamble with length $\tau_{{p}}$
(\si{\milli\second}) prior to its discovery packet (whose length is $L$
(\si{\milli\second})). The distribution of the residence times is identical
for all nodes. This process is outlined in Fig.~\ref{fig:nodeRen}.

In this mode, we will minimize the listening period and simply transmit a preamble to minimize energy consumption from listening ($\tau_l \approx 0$). Then, the renewal is that nodes sleep and then wakeup and do a quick listen to see if anyone else is transmitting. Then, if the channel is free the node will begin to transmit a preamble for a duration of time, $\tau_p$. We first consider $\tau_p$ as a stochastic period of time with rate $\lambda_p$. Then, in subsection \ref{sec:pream_det}, we consider $\tau_p$ as a deterministic time period. 

%Energy consumed per period
%$\frac{1}{F}\tau_{l} + \frac{T}{F} (\tau_p+1).$
%To analyze this model of operation, we will use techniques from renewal theory. Each node undergoes a renewal whose length of time is $\rho = \tau_s+\tau_l+\tau_p+1$. To maintain energy neutrality, IoTags must (on average) spend energy the rate of energy harvested. Hence, the energy constrain is that:


\subsection{$\tau_p \sim$ Exponential with Rate $\lambda_p$}
\label{sec:pream_exp}
In this model, the first node to finish sleeping will be the node who transmits for the renewal. As the listening period is an exponential random variable, the likelihood of one of the $N-1$ sleeping nodes waking up and listening to the transmission can easily be computed as two competing exponential random variables, $\lambda_s/(\lambda_s+\lambda_p)$. As each of the sleeping nodes are independent, the expected number of listeners is $\E[N_{rx}] = (N-1)\lambda_s/(\lambda_s+\lambda_p)$. The expected duration of the renewal is the $\rho = 1/(N \lambda_s) + 1/\lambda_p + 1$. 

\begin{align}
\text{max}_{\lambda_s, \lambda_p} & \quad  = \frac{(N-1)\lambda_s}{(\lambda_s+\lambda_p)( 1/(N \lambda_s) + 1/\lambda_p + 1)} & \label{eqn:objPreStoch}
\end{align}

\begin{equation}
\begin{aligned}
\text{subject to} & % \notag \\
\quad \frac{1}{N}(1/\lambda_p+1)\frac{T}{F} + \\
& \quad \frac{N-1}{N} (\frac{\lambda_s}{\lambda_s+\lambda_p}) (\chi+1)\frac{1}{F}&\\
& \quad =  1/(N \lambda_s) + 1/\lambda_p + 1, & \label{eqn:constraintPreDet}
\end{aligned}
\end{equation}

\subsection{$\tau_p \sim$ Deterministic}
\label{sec:pream_det}
\begin{align}
\text{max}_{\lambda_s, \tau_p} & \quad  = \frac{(N-1)(1-\mathrm{e}^{-\lambda \tau_p})}{1/(N \lambda_s) + \tau_p + 1} & \label{eqn:objPreDet}
\end{align}

\begin{equation}
\begin{aligned}
\text{subject to} & % \notag \\
\quad \frac{1}{N}(1/\lambda_p+1)\frac{T}{F} + \\
& \quad \frac{N-1}{N} (1-\mathrm{e}^{-\lambda_s \tau_p}) (\chi+1)\frac{1}{F}&\\
& \quad =  1/(N \lambda_s) +\tau_p + 1, & \label{eqn:constraintPreStoch}
\end{aligned}
\end{equation}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../mobicom2"
%%% End: 


==> tex/prelim.tex <==


\iffalse
\begin{figure}
\centering
\subfigure[Step 1: Node 1 transmits]{\includegraphics[width=0.3\columnwidth]{figs/figBidir1}}
\subfigure[Step 2: Node 2 transmits]{\includegraphics[width=0.3\columnwidth]{figs/figBidir2}}
\subfigure[Step $N$: Node $N$ transmits]{\includegraphics[width=0.3\columnwidth]{figs/figBidirK}}
\caption{\label{fig:bidir}}
\end{figure}
\fi

% Goal: perpetual nd
%The goal of the nodes is to discover one another \emph{indefinitely}. 




%We therefore

%Most works focus on minimizing the time until the initial discovery, assuming that repeated discoveries can leverage the initial information. However, for nodes powered by EH, the long sleep periods renders any coordination from an initial disocvery.

%\subsection{Bi-Directional Discovery}
\iffalse
A simple \emph{uni-directional} ND protocol is shown in Fig.~\ref{fig:bidir}(a). Node 1 broadcasts a `hello' message before going back into a sleep state and $N-1$ neighbors receive the message. As such, all of the neighboring nodes who receive the message become aware of node 1, as indicated via a directional link. However, the source node is not aware of the neighbors. In this scenario, the energy consumed by each node can be carefully controlled by adapting the rate of transmission and listening: node 1 spends energy to transmit a message and the $N-1$ neighbors spend energy to listen to a single message. 

To establish \emph{bi-directional} ND is much more complex. After the initial phase where node 1 transmits a message, node 1 must then wait for an acknowledgement. After the $N-1$ neighboring nodes receive a message, they must respond and acknowledge receipt. As such, consider the scenario just after the uni-directional phase shown in Fig.~\ref{fig:bidir}(a). The source node then enters a listening state. In an ideal scenario with conflict resolution, one of the $N-1$ neighbors (node 2) will respond with a broadcasted `hello' message as shown in Fig.~\ref{fig:bidir}(b). At this point in time, each node who successfully heard node 2 now also needs to acknowledge that receipt. Under this basic modification to establish bi-directional ND, each node will end up consuming energy for 1 transmission and $N-1$ message receptions as shown in Fig.~\ref{fig:bidir}(c).\footnote{If we consider the overhead in idle listening resulting from the clock drifts during the conflict resolution phases, the energy consumption only increases.}

Hence, establishing bi-directional neighbor discovery presents a very difficult modeling challenge as the energy consumed by a node is highly dependent on the number of neighbors who overhear the message. Note that policies which attempt to delay the acknowledgement message will only incur more energy consumption as the longer the time between the handshake, the more drift in the nodes clocks which results in added idle listening.


%\subsection{Coordination/Synchronization}
ND in IoTag networks is made challenging due to a lack of coordination which results in \emph{idle listening} and \emph{unheard transmissions}. If IoTags were coordinated, ND would simply involve waking the device at the exact moment when a message was to be heard. However, in IoTag networks there is no centralized coordination mechanism as is common in traditional wireless networks (i.e., WiFi, LTE). Therefore, devices must behave in a probabilistic manner to discover their neighbors. 

Even after an initial link establishment between two nodes, the achieved coordination/synchronization information will not benefit the ND algorithms. For one, maintaining coordination/schedule information for a node and all of his neighbors may become too complex to schedule. And in addition, the degree of coordination between neighbors degrades quickly due to the drift in clock synchronization between the devices. For example, if a source and destination agree to a transmission at some time in the future, the destination node will need to add a \emph{guard time} around the expected message receive time to account for clock drifts. In practice, the added energy consumption during the guard time can outweigh the consumption of the actual message. 

%However, this presents numerous challenges. First, recall that all nodes are homogenous and are not coordinated; hence, all of the neighboring nodes must follow the same protocol to respond to the source node. 

%\subsection{Energy Interdependency: Search vs.\ Discovery} %Controlling the rate of success
%\comment{To be determined}
IoTags have interdependency in the energy consumed between neighboring nodes; to discover a neighbor, one node must broadcast a `hello' message and a second must listen to the channel. Due to variations in transceiver energy costs to transmit and listen, this can result in variations in energy consumed.\\
\fi















%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../sensys15"
%%% End: 

